Efficient Parallel Verification of Galois Field Multipliers

Galois field (GF) arithmetic is used to implement critical arithmetic components in communication and security-related hardware, and verification of such components is of prime importance. Current techniques for formally verifying such components are based on computer algebra methods that proved successful in verification of integer arithmetic circuits. However, these methods are sequential in nature and do not offer any parallelism. This paper presents an algebraic functional verification technique of gate-level GF (2m ) multipliers, in which verification is performed in bit-parallel fashion. The method is based on extracting a unique polynomial in Galois field of each output bit independently. We demonstrate that this method is able to verify an n-bit GF multiplier in n threads. Experiments performed on pre- and post-synthesized Mastrovito and Montgomery multipliers show high efficiency up to 571 bits.

==> two_tables_side_by_side.tex <==
        \begin{minipage}{.5\linewidth}
        \small
      %\caption{$P(x)$=$x^{4}+x^{3}+1$}
      \centering
\begin{tabular}{cccc}
\multicolumn{4}{l}{$P(x)$=$x^{4}+x^{3}+1$}                                                                            \\
\multicolumn{1}{c|}{$s_3$} & \multicolumn{1}{c|}{$s_2$} & \multicolumn{1}{c|}{$s_1$} & $s_0$                     \\
\multicolumn{1}{c|}{$s_4$} & \multicolumn{1}{c|}{0}  & \multicolumn{1}{c|}{0} & $s_4$                     \\
\multicolumn{1}{c|}{$s_5$} & \multicolumn{1}{c|}{0}  & \multicolumn{1}{c|}{$s_5$}  & $s_5$                     \\
\multicolumn{1}{c|}{$s_6$} & \multicolumn{1}{c|}{$s_6$} & \multicolumn{1}{c|}{$s_6$}  & $s_6$                      \\ \hline
\multicolumn{1}{l|}{$z_3$} & \multicolumn{1}{l|}{$z_2$} & \multicolumn{1}{l|}{$z_1$} & \multicolumn{1}{l}{$z_0$}
\end{tabular}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
        %\caption{$P(x)$=$x^{4}+x+1$}
\begin{tabular}{cccc}
\multicolumn{4}{l}{$P(x)$=$x^{4}+x+1$}                                                                            \\
\multicolumn{1}{c|}{$s_3$} & \multicolumn{1}{c|}{$s_2$} & \multicolumn{1}{c|}{$s_1$} & $s_0$                     \\
\multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0}  & \multicolumn{1}{c|}{$s_4$} & $s_4$                     \\
\multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{$s_5$}  & \multicolumn{1}{c|}{$s_5$}  & 0                     \\
\multicolumn{1}{c|}{$s_6$} & \multicolumn{1}{c|}{$s_6$} & \multicolumn{1}{c|}{0}  & 0                      \\ \hline
\multicolumn{1}{l|}{$z_3$} & \multicolumn{1}{l|}{$z_2$} & \multicolumn{1}{l|}{$z_1$} & \multicolumn{1}{l}{$z_0$}
\end{tabular}    \end{minipage} 
\caption{Analysis of the computation complexity of Galois field multipliers with different irreducible polynomials using two 4-bit GF multiplications, which are implemented using $x^{4}+x^{3}+1$ and $x^{4}+x+1$.}
\vspace{-5mm}
\label{study}
\end{figure}

